Reduced rank regression for neural communication: a tutorial for neuroscientists

Reduced rank regression (RRR) is a statistical method for finding a low-dimensional linear mapping between a set of high-dimensional inputs and outputs. In recent years, RRR has found numerous applications in neuroscience, in particular for identifying "communication subspaces" governing the interactions between brain regions. This tutorial article seeks to provide an introduction to RRR and its mathematical foundations, with a particular emphasis on neural communication. We discuss RRR's relationship to alternate dimensionality reduction techniques such as singular value decomposition (SVD), principal components analysis (PCA), principal components regression (PCR), and canonical correlation analysis (CCA). We also derive important extensions to RRR, including ridge regularization and non-spherical noise. Finally, we introduce new metrics for quantifying communication strength as well as the alignment between communication axes and the principal modes of neural activity. By the end of this article, readers should have a clear understanding of RRR and the practical considerations involved in applying it to their own data.

==> jpdefs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Helpful definitions for TeX
%%%  Eero Simoncelli, 6/90.
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\long\def\comment#1{}
\long\def\nocomment#1{#1}   %to easily re-insert commented text
\long\def\mcomment#1{
	\marginpar[\singlesp\footnotesize #1 \fbox{\rule{1ex}{0ex}\rule{0ex}{1ex}}]
		  {\singlesp\footnotesize \fbox{\rule{1ex}{0ex}\rule{0ex}{1ex}} #1}}

%%% Set the spacing between lines: 1.0 means single-space.
%%% Must call a textsize command to get the new baselinestretch to
%%% work.  Thus this function resets the text size to \normalsize.
\def\setspacing#1{\renewcommand\baselinestretch{#1}\large\normalsize}

%%%  Use before 1st paragraph of a section to force an indentation.
%%% Correct solution is to redefine the sectioning commands in the
%%% appropriate style files (eg, art11.sty).
\newcommand{\yesindent}{\hspace*{\parindent}}    %%{\hskip \parindent}

\newcommand\doublesp{\renewcommand\baselinestretch{1.8}\large\normalsize}
\newcommand\singlesp{\renewcommand\baselinestretch{1.1}\large\normalsize}
\newcommand\halfsp{\renewcommand\baselinestretch{1.5}\large\normalsize}

\newenvironment{ct}
	{\begin{center}\begin{tabular}}
	{\end{tabular}\end{center}}

%%% Non-numbered subsections, with table of contents entries
\def\mychapter#1{\def\baselinestretch{1.0}\chapter{#1}\vskip 0.25in}
\def\mychap#1{\addcontentsline{toc}{chapter}{#1}
		\def\baselinestretch{1.0}\chapter*{#1}\vskip 0.25in}
\def\mysec#1{\addcontentsline{toc}{section}{$\circ$\hskip 0.4em #1}
		\section*{#1}}
\def\mysubsec#1{\addcontentsline{toc}{subsection}{$\circ$\hskip 0.4em #1} 
		\subsection*{#1}}
\def\mysubsubsec#1{\addcontentsline{toc}{subsubsection}{$\circ$\hskip 0.4em #1}
		\subsubsection*{#1}}

%%% A macro for figures to be MANUALLY pasted.  The arguments are the figure
%%% height, the figure label, and the figure caption.  The macro makes
%%% space for the figure, prints the label in center of the space (as
%%% an identifier), and prints the caption.
\long\def\myfig#1#2#3{
	\vbox to #1{\vfil \center{#2} \vfil} %Print label in box
	\caption{#3}
	\label{#2}}

%%% Macro for vertically aligning a subfigure and its label.
%%% Example usage: \sublabel{(a)}{\psfig{ ... }}
\def\sublabel#1#2{ \begin{tabular}{c} #2 \\  #1 \end{tabular}}

%%% New version of \caption puts things in smaller type, single-spaced 
%%% and indents them to set them off more from the text.
\makeatletter
\long\def\@makecaption#1#2{
	\vskip 0.8ex
	\setbox\@tempboxa\hbox{\small {\bf #1:} #2}
        \parindent 1.5em  %% How can we use the global value of this???
	\dimen0=\hsize
	\advance\dimen0 by -3em
	\ifdim \wd\@tempboxa >\dimen0
		\hbox to \hsize{
			\parindent 0em
			\hfil 
			\parbox{\dimen0}{\def\baselinestretch{0.96}\small
				{\bf #1.} #2
				%%\unhbox\@tempboxa
				} 
			\hfil}
	\else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
	\fi
	}
\makeatother

%%%% original version of caption
%\long\def\@makecaption#1#2{
%   \vskip 10pt 
%   \setbox\@tempboxa\hbox{#1: #2}  
%   \ifdim \wd\@tempboxa >\hsize   % IF longer than one line:
%       \unhbox\@tempboxa\par      %   THEN set as ordinary paragraph.
%     \else                        %   ELSE  center.
%       \hbox to\hsize{\hfil\box\@tempboxa\hfil}  
%   \fi}

%%% Footnotes without numbers, modified from latex.tex definition of
%%% footnotetext.  NOTE: Can use \thanks if doing this on the title
%%% page. 
\makeatletter
\long\def\barenote#1{
    \insert\footins{\footnotesize
    \interlinepenalty\interfootnotelinepenalty 
    \splittopskip\footnotesep
    \splitmaxdepth \dp\strutbox \floatingpenalty \@MM
    \hsize\columnwidth \@parboxrestore
    {\rule{\z@}{\footnotesep}\ignorespaces
	      % indent
      #1\strut}}}
\makeatother

\def\bulletnote#1{\barenote{$\bullet$ #1}}
        
%%% Math definitions:
%\newtheorem{prop}{Proposition}
%\newenvironment{proof}{{\sl Proof: }}{\rule{0.07in}{0.13in}}

%%%p.100 Latex for \fbox with \rule
%%%Hollow: {\fbox{\rule{0.07in}{0in}\rule{0in}{0.14in}}}

%%% Inserting text into multi-line formulas.  See p. 193, Tex manual.
%%% Can also use \rm \noindent instead of \hbox, allowing longer lines.
%%\def\mtext#1{\noalign{\hbox{#1} \smallskip \medskip}}
\long\def\mtext#1{\noalign{\rm \noindent{#1}}}

%%% Insert space after or before or in an equation
%% \vbox to \medskipamount{\vfil}
%\def\eqsmallskip{\hbox{\smallskip }\nonumber\\}
%\def\eqmedskip{\hbox{\medskip} \nonumber \\}  
%\def\eqbigskip{\hbox{\bigskip} \nonumber \\} 
\def\eqsmallskip{\rule[\baselineskip]{0pt}{\smallskipamount}}
\def\eqmedskip{\rule[\baselineskip]{0pt}{\medskipamount}}
\def\eqbigskip{\rule[\baselineskip]{0pt}{\bigskipamount}}

%%% Alternative: use a strut (see p. 100 of LaTeX manual)

%%% Display fraction in textstyle (ie, with slash rather than
%%% horizontal bar)
\def\sfrac#1#2{{\textstyle \frac{#1}{#2}}}   

%% Format in tabbing (paragraph) mode, producing a box that is shrunk
%% to fit the paragraph.  First arg is margin, second is paragraph.
%% NOTE: minipage of tabbing fits paragraph, see LaTeX, p. 100.
\makeatletter
\long\def\shrinkbox{\@ifnextchar[{\@mgnshrinkbox}{\@shrinkbox}}

\def\@shrinkbox#1{
	\begin{minipage}{\columnwidth}\begin{tabbing}
	#1
	\end{tabbing}\end{minipage}}

\def\@mgnshrinkbox[#1]#2{
   \setbox\@tempboxa\hbox{\unskip\begin{minipage}{\columnwidth}\begin{tabbing}
		#2
		\end{tabbing}\end{minipage}\unskip}
   \dimen0=\wd\@tempboxa
   \advance\dimen0 by #1
   %%\advance\dimen0 by #1
   \dimen1=\ht\@tempboxa
   \advance\dimen1 by #1
   \advance\dimen1 by #1
   \makebox[\dimen0]{\vbox to \dimen1{\vfil \box\@tempboxa \vfil}}}
\makeatother

%  \F for the Fourieroperator
\newcommand{\F}{\mbox{$\cal F$}}

%  \R and \C   The set of Real and Complex numbers
%  may be used in equation or text mode
%  LaTeX has \Re but no \Co; define both in the traditional form (non script)
%\newcommand{\R}{\mbox{\rule[0ex]{.2ex}{1.56ex} \hspace{-1.6ex} \bf R}}
\newcommand{\R}{\mbox{I \hspace{-2ex} {\bf R}}} 
\newcommand{\C}{\mbox{   % mbox removes italics in equation mode
                \rule[.125ex]{0ex}{1.1ex}  % take out second line for now
                \hspace{-1.2ex}
                \rule[.0625ex]{.2ex}{1.4ex}
                \hspace{-2.4ex}
                \bf C
                }}
\newcommand{\Z}{\mbox{Z\hspace{-2ex}{\bf Z}}}

\def\etal{{\sl et~al.}}

%new caption macro
\makeatletter
\long\def\@makecaption#1#2{
        \vskip 10pt
        \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
        \parindent 1.5em  %% How can we use the global value of this???
        \dimen0=\hsize
        \advance\dimen0 by -2\parindent
        \ifdim \wd\@tempboxa >\dimen0
                \hbox to \hsize{
                        \hfil
                        \parbox{\dimen0}{\def\baselinestretch{1.05}\small
                                {\bf #1:} #2
                                %%\unhbox\@tempboxa
                                }
                        \hfil}
        \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
        \fi}
\makeatother

% ============================================================
% More macros (jpdefs.tex)

\newcommand{\asection}[1]{
        \addtocounter{section}{1}
        \setcounter{subsection}{0}
        \section*{Appendix \Alph{section}: #1}
        \addcontentsline{toc}{section}{Appendix \Alph{section}: #1}}

\newcommand{\asubsection}[1]{
        \addtocounter{subsection}{1}
        \subsection*{\Alph{section}.\arabic{subsection} #1}
\addcontentsline{toc}{subsection}{\Alph{section}.\arabic{subsection} #1}}
\newcommand{\asubsubsection}[1]{
        \addtocounter{subsubsection}{1}
        \subsection*{\Alph{section}.\arabic{subsection}. .\arabic{subsubsection} #1}
\addcontentsline{toc}{subsection}{\Alph{section}.\arabic{subsection}.\arabic{subsubsection} #1}}


\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}

% ---------- Symbols for ``Reals'', ``Complex Numbers'', etc. ----
\newcommand{\Reals}{{\sf R\hspace*{-0.9ex}\rule{0.15ex}%
{1.5ex}\hspace*{0.9ex}}}
\newcommand{\N}{{\sf N\hspace*{-1.0ex}\rule{0.15ex}%
{1.3ex}\hspace*{1.0ex}}}
\newcommand{\Q}{{\sf Q\hspace*{-1.1ex}\rule{0.15ex}%
{1.5ex}\hspace*{1.1ex}}}
\newcommand{\Complexs}{{\sf C\hspace*{-0.9ex}\rule{0.15ex}%
{1.3ex}\hspace*{0.9ex}}}


% --- Standard Math definitiones -----
\newcommand{\RR}{I\!\!R} %real numbers 
\newcommand{\Nat}{I\!\!N} %natural numbers 
\newcommand{\CC}{I\!\!\!\!C} %complex numbers

% ------- Others -------------------------------
\newcommand{\deriv}[2]{\frac{d #1}{d #2}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\D}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\DD}[2]{\frac{\partial ^2 #1}{\partial #2 ^2}}
\newcommand{\Di}[2]{\frac{\partial ^i #1}{\partial #2 ^i}}
\newcommand{\evalat}[1]{\left.#1\right|}
\newcommand{\parderiv}[2]{\frac{\partial #1}{\partial{#2}}}
\newcommand{\parDeriv}[3]{\frac{\partial^{#3} #1}{\partial{#2}^{#3}}}
\newcommand{\parwrt}[1]{\frac{\partial}{\partial{#1}}}
\newcommand{\parpowrt}[2]{\frac{\partial^{#1}}{\partial {#2}^{#1}}}
\newcommand{\partwowrt}[2]{\frac{\partial^{2}}{\partial {#2} \partial{#1}}}
\newcommand{\inv}{^{-1}}
\newcommand{\trp}{{^\top}} % transpose
\newcommand{\onehlf}{\frac{1}{2}}
\newcommand{\tonehlf}{\tfrac{1}{2}}
\renewcommand{\eqref}[1]{eq.~\ref{eq:#1}}
\newcommand{\Nrm}{\mathcal{N}}
\newcommand{\Tr}{\mathrm{Tr}}
\renewcommand{\inv}{^{-1}}
%\newcommand{\evalat}[1]{\left.#1\right|}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\renewcommand{\eqref}[1]{eq.~\ref{eq:#1}}
\newcommand{\figef}[1]{Fig.~\ref{fig:#1}}

